Importance Weighted Expectation-Maximization for Protein Sequence Design

Designing protein sequences with desired biological function is crucial in biology and chemistry. Recent machine learning methods use a surrogate sequence-function model to replace the expensive wet-lab validation. How can we efficiently generate diverse and novel protein sequences with high fitness? In this paper, we propose IsEM-Pro, an approach to generate protein sequences towards a given fitness criterion. At its core, IsEM-Pro is a latent generative model, augmented by combinatorial structure features from a separately learned Markov random fields (MRFs). We develop an Monte Carlo Expectation-Maximization method (MCEM) to learn the model. During inference, sampling from its latent space enhances diversity while its MRFs features guide the exploration in high fitness regions. Experiments on eight protein sequence design tasks show that our IsEM-Pro outperforms the previous best methods by at least 55% on average fitness score and generates more diverse and novel protein sequences.

==> 003method_old.tex <==
In this section, we introduce our method. 
First we define the problem.
Then we introduce the overall model architecture, through which we can obtain a proposal distribution from which the sampled proteins are both realistic and desirable. 
Then we describe the Monte Carlo EM in detail to optimize our model.
Next we incorporate additional features learned from the homogeneous protein sequences through Markov Random Field to constrain the path where the model climbs over the protein fitness landscape, to faster find the satisfactory candidates.
Finally We give a theoretical justification to prove that the designed protein sequences from the proposal distribution are highly likely sampled from the target conditional distribution.

\subsection{Problem Definition}
% Our goal is to search over a space of discrete protein sequences $\mathcal{C}^{L}$ where $\mathcal{C}$ belongs to the 20 amino acids and $L$ is the sequence length, to find an object $X \in \mathcal{C}^{L}$ that maximizes a given usefulness measure (oracle) $f: \mathcal{C}^{L} \rightarrow \mathbb{R}$ \cite{brookes2019conditioning,jain2022biological,ren2022proximal}. 
Our goal is to search over a space of discrete protein sequences $\mathcal{C}^{L}$ where $\mathcal{C}$ belongs to the 20 amino acids and $L$ is the sequence length, to find an object $X \in \mathcal{C}^{L}$ that maximizes a given oracle model \cite{brookes2019conditioning,jain2022biological,ren2022proximal}. 
We consider the setting where the oracle model provides a likelihood function $P_d(Y|X)$ over the fitness Y (typically a real-valued property for a specific protein), given a particular protein sequence X.
Then the probability $P(Y\ge\gamma | X)=1- \int_{- \infty}^{\gamma} P_d(Y|X)dY$ denotes how possible the fitness of a given protein sequence is larger than a threshold $\lambda$.
Accordingly, our task can be defined as:
\begin{equation}
X^* = \argmax_{X \in \mathcal{C}^{L}} P(Y\ge\gamma | X)P_{\theta}(X)
\label{equation1}
\end{equation}
where $P_{\theta}(X)$ is the generative model trained on the protein sequences from the same family. To simplify the expression, we representing $Y\ge \gamma$ with $\mathbb{S}$, and our objective can be reformulated as:
\begin{equation}
X^* = \argmax_{X \in \mathcal{C}^{L}} P(\mathbb{S} | X)P_{\theta}(X)
\label{equation2}
\end{equation}

\subsection{Overall Training Objective}
The ultimate goal is to design satisfactory protein sequences which should be both realistic and have high property values within a tolerant search cost.
However, if we randomly search the candidate space according to the objective in Equation \ref{equation2}, the time cost would be intensive as the search space is really large (O($20^L$)).
Thus, directly sampling good candidates from a target distribution $P_{\theta}(X|\mathbb{S})$ which takes both fitness necessity and underlying data distribution into consideration seems a good choice:
\begin{equation}
\small 
P_{\theta}(X|\mathbb{S})=\frac{P_{\theta}(X)P(\mathbb{S}|X)}{P_{\theta}(\mathbb{S})}
\end{equation}

However, realizing this idea is difficult as computing $P_{\theta}(\mathbb{S})=\int_X P(\mathbb{S}|X)P_{\theta}(X)dX$ needs an integration over all the possible X, which is intractable.
Instead, we propose to learn a proposal model $Q_{\phi}(X)$ with learnable parameter $\phi$ to approximate $P_{\theta}(X|\mathbb{S})$.
In order to find the optimal $\phi$ of the proposal model, we choose to minimize the KL divergence between the target conditional distribution $P_{\theta}(X|\mathbb{S})$ and proposal model $Q_{\phi}(X)$:
\begin{equation}
\small
\begin{split}
\phi^* &= \argmin_{\phi} D_{KL}(P_{\theta}(X|\mathbb{S})||Q_{\phi}(X)) \\
&= \argmax_{\phi} E_{P_{\theta}(X|\mathbb{S})} \log Q_{\phi}(X) + \mathcal{H(P_{\theta})} \\
&= \argmax_{\phi} E_{Q_{\phi}(X)} [\frac{P_{\theta}(X|\mathbb{S})}{Q_{\phi}(X)} \log Q_{\phi}(X)] \\
&= \argmax_{\phi} E_{Q_{\phi}(X)} [w(X) \log Q_{\phi}(X)
\end{split}
\label{equation4}
\end{equation}
where $\mathcal{H(P_{\theta})}=-E_{P_{\theta}(X|\mathbb{S})} \log P_{\theta}(X|\mathbb{S})$ is the entropy of $P_{\theta}(X|\mathbb{S})$ and it can be dropped in the third equality because it does not matter $\phi$.
We introduce $Q_{\phi} (X)$ as an Importance Sampling proposal distribution \cite{neal2001annealed} in the third equality the unormalized importance weight $w(X)=\frac{P_{\theta}(X|\mathbb{S})}{Q_{\phi}(X)}$  since we can not directly sample from $P_{\theta}(X|\mathbb{S})$.
The above objective can be approximated through monte carlo sampling \cite{hastings1970monte,neal2001annealed}.

% &= \argmax_{\phi} E_{Q_{\phi}(X)} [\frac{P_{\theta}(X)}{Q_{\phi}(X)}P(\mathbb{S}|X) \log Q_{\phi}(X)] \\

We can prove that under an acceptable KL distance, the samples from the proposal distribution $Q_{\phi}(X)$ can be bound within a reasonable sampling error from the target distribution $P_{\theta}(X|\mathbb{S})$.

\begin{lemma}
If the KL divergence between two distributions P and Q is less than a small positive value $\delta$, then the sampling probability difference between P and Q will be bounded by $\sqrt{2\delta}$ for each sample x.
\end{lemma}
\begin{proof}\renewcommand{\qedsymbol}{}
Let $\delta(P, Q)$ be the total variation distance between P and Q, due to the Pinsker's inequality \cite{csiszar2011information}, we have 
\begin{equation}
\small
\frac{1}{2}\sum_{x} |P(x)-Q(x)| = \delta(P, Q) \le \sqrt{\frac{1}{2} D_{KL}(P||Q)} < \sqrt{\frac{1}{2}\delta}
\label{pinsker}
\end{equation}
\end{proof}
The first equality in Equation \ref{pinsker} holds when the measurable space is discrete as is the case here.
The second equality holds if and only if $P=Q$, and then there is no difference in sampling from $P$ and $Q$.
Thus, we can get:
\begin{equation}
\small
\sum_{x} |P(x)-Q(x)| < \sqrt{2\delta}
\end{equation}
When $\delta$ approaches $0$, the sampling difference between $P(x)$ and $Q(x)$ would be very minor. 

% In information theory, the entropy $H_{\theta}=-E_{P_{\theta}(X|\mathbb{S})} \log P_{\theta}(X|\mathbb{S})$ of $P_{\theta}(X|\mathbb{S})$ is a lower bound of the cross-entropy between $P_{\theta}(X|\mathbb{S})$ and $Q_{\phi}(X)$ because:
% \begin{equation}
% \begin{split}
% \log \int_X Q_{\phi}(X) &= \log \int_X P_{\theta}(X|\mathbb{S}) \frac{Q_{\phi}(X)}{P_{\theta}(X|\mathbb{S})} \\
% & \ge E_{P_{\theta}(X|\mathbb{S})} \log Q_{\phi} (X) + H_{\theta}
% \end{split}
% \label{equation4.1}
% \end{equation}
% where the second lower bound is due to Jensen's Inequality. Thus, we can obtain the constraint function of $Q_{\phi} (X)$:
% \begin{equation}
% -E_{P_{\theta}(X|\mathbb{S})} \log Q_{\phi} (X) \ge H_{\theta}
% \end{equation}
% The above equality holds if and only if $Q_{\phi} (X)=P_{\theta}(X|\mathbb{S})$.

% But directly sampling from $P_{\theta}(X|\mathbb{S})$ is difficult as:
% \begin{equation}
% P_{\theta}(X|\mathbb{S})=\frac{P_{\theta}(X)P(\mathbb{S}|X)}{P_{\theta}(\mathbb{S})}
% \end{equation}
% where computing $P_{\theta}(\mathbb{S})=\int_X P(\mathbb{S}|X)P_{\theta}(X)dX$ needs an integration over all the possible X, which is intractable.
% Instead, we propose to learn a search model $Q_{\phi}(X)$ to approximate $P_{\theta}(X|\mathbb{S})$ where $\phi$ is the learnable parameter.
% To find the optimum $\phi$ of the search model, we can minimize the KL divergence between the target conditional $P_{\theta}(X|\mathbb{S})$ and search model $Q_{\phi}(X)$:
% \begin{equation}
% \begin{split}
% \phi^* &= \argmin_{\phi} KL(P_{\theta}(X|\mathbb{S})||Q_{\phi}(X)) \\
% &= \argmax_{\phi} E_{P_{\theta}(X)} [P(\mathbb{S}|X) \log Q_{\phi}(X)]
% \end{split}
% \label{equation4}
% \end{equation}
% Since $\mathbb{S}$ is usually a rare event, $P(\mathbb{S}|X)$ may be very small, which may lead to issues in model training. We instead use importance sampling to avoid this issue, and the optimize objective becomes:
% \begin{equation}
% \begin{split}
% \phi^* &= \argmax_{\phi} E_{Q_{\phi}(X)} [\frac{P_{\theta}(X)}{Q_{\phi}(X)}P(\mathbb{S}|X) \log Q_{\phi}(X)] \\
% &= \argmax_{\phi} E_{Q_{\phi}(X)} [w(X) \log Q_{\phi}(X)]
% \end{split}
% \label{equation5}
% \end{equation}
% where $w(X)=\frac{P_{\theta}(X)}{Q_{\phi}(X)}P(\mathbb{S}|X)$.
% The above objective can be approximated through Monte Carlo sampling.

\subsection{Importance Sampling based EM}
Diversity is a key consideration in our protein design procedure, which can not only increase the success rate of the traditional directed evolution pipeline, but also satisfy the diverse nature in species.
Due to this consideration, we incorporate latent variables into our model to promote diverse protein generation, which has been proven effective in many text generation tasks \cite{semeniuta2017hybrid,wang2019topic}.
In general, variational inference is a difficult non-convex optimization problem, typically requiring a lengthy iterative estimation procedure. 
% However, standard inference models attempt to perform this optimization through a discriminative mapping from data observations to approximate posterior parameters \cite{marino2018iterative}. This often leads to a sub-optimal estimation as shown in Figure \ref{figure2} (b).
Therefore, we employ variational EM to optimize our proposal model, of which the iterative process can not only lead to a better estimate (Figure \ref{figure2} (b)) but also naturally fulfill the iterative protocol in traditional directed evolution methods.

Specifically, starting from our training objective in Equation \ref{equation4}, we incorporate a latent variable $Z$,
\begin{equation}
\small 
\begin{split}
\phi^* &= \argmax_{\phi} E_{Q_{\phi}(X)} [\frac{P_{\theta}(X|\mathbb{S})}{Q_{\phi}(X)} \log Q_{\phi}(X)] \\
&= \argmax_{\phi} E_{Q_{\phi}(X, Z)} [\frac{P_{\theta}(X, Z| \mathbb{S})}{Q_{\phi}(X, Z)} \log Q_{\phi}(X)]  \\
&= \argmax_{\phi} E_{Q_{\phi}(X, Z)} [\frac{P_{\theta}(X,Z)}{Q_{\phi}(X,Z)}P(\mathbb{S}|X) \log Q_{\phi}(X)] 
\end{split}
\label{equation_em}
\end{equation}
The second equality in Equation \ref{equation_em} holds due to the fact that an expectation over a marginal distribution is equal to the same expectation over an augmented joint distribution, i.e., $E_{p(x)}[f(x)]=E_{p(x,y)}[f(x)]$.
The third equality holds since $P_{\theta}(X, Z| \mathbb{S})=\frac{P_{\theta}(X,Z)P(\mathbb{S}|X)}{P_{\theta}(\mathbb{S})}$ and $P_{\theta}(\mathbb{S})$ does not rely on $\phi$.

Here we share the prior $P(Z)$ for $P_{\theta}(X,Z)$ and $Q_{\phi}(X, Z)$, and thus the above objective becomes:
\begin{equation}
\small
\phi^* = \argmax_{\phi} E_{Q_{\phi}(X, Z)} [\frac{P_{\theta}(X|Z)}{Q_{\phi}(X|Z)}P(\mathbb{S}|X) \log Q_{\phi}(X)] 
\label{equation7}
\end{equation}
Applying the iterative protocol in EM, the above optimization objective can be reformulated as:\\
\begin{equation}
\small 
\begin{split}
\phi^{(t+1)} &= \argmax_{\phi} E_{Q_{\phi^{(t)}}(X, Z)} [\frac{P_{\theta}(X|Z)}{Q_{\phi^{(t)}}(X|Z)}P(\mathbb{S}|X) \log Q_{\phi}(X)]  \\
&= \argmax_{\phi} E_{Q_{\phi^{(t)}}(X, Z)} [w(X^{(t)}, Z^{(t)}) \log Q_{\phi}(X)]
\end{split}
\label{equation9}
\end{equation}
where $w(X^{(t)}, Z^{(t)}) =  \frac{P_{\theta}(X|Z)}{Q_{\phi^{(t)}}(X|Z)}P(\mathbb{S}|X)$.
At iteration $t$, the internal log marginal likelihood can be reformulated as the predefined EM objective:
\begin{equation}
\small
\begin{split}
\log Q_{\phi}(X) &= \log \int_Z Q_{\phi} (X, Z) dZ \\
&= \log \int_Z Q_{\phi^{(t)}}(Z) \frac{Q_{\phi} (X, Z)}{Q_{\phi^{(t)}}(Z)} dZ \\
&= E_{Q_{\phi^{(t)}}(Z)} [\log Q_{\phi}(X, Z) -\log Q_{\phi^{(t)}}(Z)] \\&+ D_{KL}(Q_{\phi^{(t)}}(Z)||Q_{\phi}(Z|X))\\
&= \mathcal{F}(Q_{\phi^{(t)}}(Z), Q_{\phi}(X, Z))
\end{split}
\end{equation}
Then the optimization process can be reformulated as :\\
E-step: set $Q_{\phi^{(t+1)}}(Z)=Q_{\phi^{(t)}}(Z|X)$\\
M-step: \\
\begin{equation}
\small 
\begin{split}
\phi^{(t+1)} = \argmax_{\phi} \;& E_{Q_{\phi^{(t)}}(X, Z)} \{w(X^{(t)}, Z^{(t)}) \\&\boldsymbol{\cdot} \mathcal{F}(Q_{\phi^{(t+1)}}(Z), Q_{\phi}(X, Z))\}
\end{split}
\end{equation}
The M-step can be approximated through the importance sampling with joint samples $(X_i, Z_i) \sim Q_{\phi^{(t)}}(X, Z)$:
\begin{equation}
\small
\phi^{(t+1)} = \argmax_{\phi} \frac{\sum_{i=i}^N w(X_i, Z_i) \mathcal{F}(Q_{\phi^{(t+1)}}(Z_i), Q_{\phi}(X_i, Z_i))}{\sum_{i=i}^N w(X_i, Z_i)}
\label{importance_final}
\end{equation}

Through this iterative process, we can obtain a good proposal distribution $Q_{\phi}$, from which we can directly sample satisfactory candidates with small time cost.

\subsection{Learning Constraints from Homogeneous Sequences}
As shown in previous work, amino acid inter-dependencies can be learned from a generative graphical model Markov Random Field (MRF) fitted on the sequences from the same family, to uncover the underlying constraints that define the family \cite{hopf2017mutation,luo2021ecnet}.
These constraints are the results of the evolutionary process under natural selection and may reveal clues on which amino-acid combinations are more favorable than others. 
Thus, we incorporate these constraints into our model to constrain the proposal model climb over the protein landscape so as to find a faster uphill path to the desired proteins in the iterative protocol.

Specifically, the generative model generates a sequence $X=(x_1, x_2, .., x_L)$ with probability $P(X)=\frac{\exp(E(X))}{Z}$, where Z is a normalization constant. E(X) is the ‘energy function’ of sequence X in the generative model, which is defined as the sum of all pairwise coupling constraints $\varepsilon_{ij}$ and single-site constraints $\varepsilon_i$, where i and j are position indices along the protein sequence as illustrated in Figure \ref{figure3}:
\begin{equation}
\small
E(X) = \sum_{i=1}^L \varepsilon_i(x_i) + \sum_{i=1}^L\sum_{j=1, j\ne i}^L \varepsilon_{ij}(x_i, x_j)
\end{equation}
We train the model following CCMpred \cite{seemayer2014ccmpred} using a pseudo-likelihood. 
But different from them, we additionally add a lasso regularizer to the training objective to make the graph sparse, of which the regularization coefficients are set to the same values as the ones in ridge regularizer:
\begin{equation}
\small 
\begin{split}
L&=\sum_X \log P(X) - \mathcal{L}(\varepsilon) - \mathcal{R}(\varepsilon) \\
\mathcal{L}(\varepsilon) &= \lambda_{\text{single}} \sum_{i=1}^L ||\varepsilon_i||_1^1 + \lambda_{\text{pair}}\sum_{i,j=1,i\ne j}||\varepsilon_{ij}||_1^1 \\
\mathcal{R}(\varepsilon) &= \lambda_{\text{single}} \sum_{i=1}^L ||\varepsilon_i||_2^2 + \lambda_{\text{pair}}\sum_{i,j=1,i\ne j}||\varepsilon_{ij}||_2^2 \\
\end{split}
\end{equation}
Following \cite{kamisetty2013assessing}, we set $\lambda_{\text{single}}=1$ and $\lambda_{\text{pair}}=0.2*(L-1)$.

\begin{figure}
  \centering
  \includegraphics[width=7.0cm]{MRF.pdf}
  \caption{Learning constraints from homogeneous sequences.}
  \label{figure3}
\end{figure}

After training the MRF model, we can encode a protein sequence with the learned constraints. Specifically, we encode the i-th amino acid by concatenating its corresponding single-site constraints as well as the possible coupling ones as:
\begin{equation}
\varepsilon(x_i)=[\varepsilon_i(x_i), \varepsilon_{i1(x_i, a_{1\boldsymbol{\cdot}})}, \varepsilon_{i2(x_i, a_{2\boldsymbol{\cdot}})}, ..., \varepsilon_{iL(x_i, a_{L\boldsymbol{\cdot}})}] 
\end{equation}
where for any position $j \ne i$, $\varepsilon_{ij(x_i, a_{j\boldsymbol{\cdot}})}$ gathers all possible amino acids as follows:
\begin{equation}
\varepsilon_{ij(x_i, a_{j\boldsymbol{\cdot}})} = [\varepsilon_{ij(x_i, a_1)}, \varepsilon_{ij(x_i, a_2)}, ..., \varepsilon_{ij(x_i, a_{20})}]
\end{equation}
Then for each amino acid, we first map $\varepsilon(x_i)$ to the embedding space, and then add it to the original amino-acid embedding to get the final feature vector as the model input.
The optimization objective finally becomes:\\
E-step: set $Q_{\phi^{(t+1)}}(Z)=Q_{\phi^{(t)}}(Z|X, \varepsilon)$\\
% \begin{equation}
% \small 
% \begin{split}
% Q_{\phi^{(t+1)}}(Z|X, \varepsilon) &= \argmax_{Q_{\phi^{(t)}}(Z|X, \varepsilon)} E_{Q_{\phi^{(t)}}(X, Z|\varepsilon)} \{w^{(t)}(X)\\ &\cdot \mathcal{F}(Q_{\phi^{(t)}}(Z|X, \varepsilon), Q_{\phi^{(t)}}(X, Z| \varepsilon))\}
% \end{split}
% \label{equation17}
% \end{equation}
M-step: \\
\begin{equation}
\small 
\begin{split}
\phi^{(t+1)} = \argmax_{\phi} \;& E_{Q_{\phi^{(t)}}(X, Z|\varepsilon)} \{w(X^{(t)}, Z^{(t)}) \\&\boldsymbol{\cdot} \mathcal{F}(Q_{\phi^{(t+1)}}(Z), Q_{\phi}(X, Z|\varepsilon))\}
\end{split}
\label{final_em_contraint}
\end{equation}
where $\varepsilon$ are the learned constraints, and fixed here.

